Systematics of supernumerary nuclear rainbow in inelastic $^{16}$O+$^{12}$C scattering

We perform a systematic study of inelastic nuclear rainbow scattering for the \oc system to the 2$^+$ (4.44 MeV) state of $^{12}$C at incident energies of 100--608 MeV with the coupled-channels method. The recently generalized nearside-farside decomposition for inelastic scattering was applied in combination with the multichannel deflection function analysis to elucidate the origin of the nuclear rainbow phenomenon and the suppression of the primary and supernumerary Airy minima in the inelastic scattering cross section. The systematic evolution of the Airy minima for the excited 2$^+$ (4.44 MeV) state of $^{12}$C was unambiguously determined. Our work suggests that there is no clear shift in the positions of the first Airy minima and a small shift at low energies for the second and third Airy minima between the inelastic and elastic scattering cross sections. Using the $K$-subamplitudes splitting technique combined with the generalized nearside-farside decomposition and deflection function, the distinct refractive pattern commonly suppressed in the inelastic heavy-ion scattering can be interpreted and provides new insights into the relationship between elastic and inelastic nuclear rainbow scattering.

==> biold.tex <==
\begin{thebibliography}{99}
\bibitem{Sa79} G.R. Satchler and W.G. Love, Phys. Rep. {\bf 55}, 183 (1979).
\bibitem{Bra97} M.E. Brandan and G.R. Satchler, Phys. Rep. {\bf 285}, 143 (1997).
\bibitem{Kho07r} D.T. Khoa, W. von Oertzen, H.G. Bohlen, and S. Ohkubo,
 J. Phys. G {\bf 34}, R111 (2007).
\bibitem{Hus84}M.S. Hussein and K.W. McVoy, Prog. Part. Nucl. Phys. {\bf 12}, 103 (1984).
\bibitem{Bra96} M.E. Brandan, M.S. Hussein, K.W. McVoy, and G.R. Satchler, 
	{\it Comments on nuclear and particle physics}, Vol.~22 (Gordon and Breach, 
	New York, 1996), p.~77. 
\bibitem{Fri88} S.H. Fricke, M.E. Brandan, and K.W. McVoy,
	Phys. Rev. C {\bf 38}, 682 (1988).
\bibitem{Bri77} D.M. Brink and N. Takigawa, Nucl. Phys. A {\bf 279}, 159 (1977).
\bibitem{Row77} N. Rowley, H. Doubre, and C. Marty, Phys. Lett. B {\bf 69}, 
 147 (1977).
\bibitem{Ful75} R.C. Fuller, Phys. Rev. C {\bf 12}, 1561 (1975).
\bibitem{Kho16} D.T. Khoa, N.H. Phuc, D.T. Loan, and B.M. Loc,
	Phys. Rev. C {\bf 94}, 034612 (2016).
\bibitem{Kho00} D.T. Khoa, W. von Oertzen, H.G. Bohlen, and F. Nuoffer, 
 Nucl. Phys. A {\bf 672}, 387 (2000).
\bibitem{Mcv92} K.W. McVoy and M.E. Brandan, Nucl. Phys. A {\bf 542},
 295 (1992).
\bibitem{Sto79} R.G. Stokstad, R.M. Wieland, G.R. Satchler, C.B. Fulmer,
 D.C. Hensley, S. Raman, L.D. Rickertsen, A.H. Snell, and P.H. Stelson,
 Phys. Rev.  C {\bf  20}, 655 (1979).
\bibitem{Sti89} E. Stiliaris, H. G. Bohlen, P. Fr\"obrich, B. Gebauer, D. Kolbert, 
 W. von Oertzen, M. Wilpert, and Th. Wilpert, Phys. Lett. B {\bf 223}, 291 (1989).
\bibitem{Sat83} G.R. Satchler, {\it Direct Nuclear Reactions} (Clarendon, Oxford, 1983).
\bibitem{Phuc21} N.H. Phuc, D.T. Khoa, and N.T.T. Phuc,  
Eur. Phys. J. A {\bf 57}, 75 (2021). 
%---------------------------elastic OC data---------------------------
\bibitem{Bra91} M.E. Brandan and G.R. Satchler, Phys. Lett. B {\bf 256}, 311 (1991).
\bibitem{Rou85} P. Roussel, N. Alamanos, F. Auger, J. Barrette, B. Berthier, 
 B. Fernandez, L. Papineau, H. Doubre, and W. Mittig, Phys. Rev. Lett. {\bf 54}, 1779 (1985).
\bibitem{Bra86} M.E. Brandan, A. Menchaca-Rocha, M. Buenerd, J. Chauvin, 
 P. De Saintignon, G. Duhamel, D. Lebrum, P. Martin, G. Perrin, and J.Y. Hostachy, 
 Phys. Rev. C {\bf 34}, 1484 (1986). 
\bibitem{Vil89} A.C.C. Villari, A. L\'{e}pine-Szily, R.L. Filho, O.P. Filho, M.M. Obuti, 
 J.M. Oliveira Jr, and N. Added, Nucl. Phys. A  {\bf 501}, 605 (1989).
\bibitem{Oglo98} A.A. Ogloblin, D.T. Khoa, Y. Kond\=o, Yu.A. Glukhov, 
 A.S. Demyanova, M.V. Rozhkov, G.R. Satchler, and S.A. Goncharov, 
 Phys. Rev. C {\bf 57}, 1797 (1998). 
\bibitem{Oglo00} A.A. Ogloblin, Yu.A. Glukhov, W.H. Trzaska, A.S. Demyanova, 
	S.A. Goncharov, R. Julin, S.V. Klebnikov, M. Mutterer, M.V. Rozhkov, 
	V.P. Rudakov, G.P. Tiorin, D.T. Khoa, and G.R. Satchler, 
	Phys. Rev. C {\bf 62}, 044601 (2000).
\bibitem{Glu01-181} Yu. A. Glukhov, S.A. Goncharov, A.S. Demyanova, A.A. Ogloblin, 
 M.V. Rozhkov, V.P. Rudakov, and V. Trashka, 
 Izv. Ross. Akad. Nauk, Ser. Fiz. {\bf 65}, 647 (2001).
\bibitem{Glu07} Yu. A. Glukhov, V. P. Rudakov, K. P. Artemov, A. S. Demyanova, 
 A. A. Ogloblin, S. A. Goncharov, and A. Izadpanakh, Phys. At. Nucl. {\bf 70}, 1 (2007). 
\bibitem{Nico00} M.P. Nicoli, F. Haas, R.M. Freeman, S. Szilner, Z. Basrak, A. Morsad, 
 G.R. Satchler, and M. E. Brandan, Phys. Rev. C  {\bf 61}, 034609 (2000).
\bibitem{Bra01} M. E. Brandan, A. Menchaca-Rocha, L. Trache, H.L. Clark,
	A. Azhari, C. A. Gagliardi, Y.-W. Lui, R. E. Tribble, R. L. Varner,
	J. R. Beene, and G. R. Satchler, Nucl. Phys. A {\bf 688}, 659 (2001).
\bibitem{Kho94} D.T. Khoa, W. von Oertzen, and H.G. Bohlen, 
 Phys. Rev. C {\bf 49}, 1652 (1994).
\bibitem{Kho97} D.T. Khoa, G.R. Satchler, and W. von Oertzen,
 Phys. Rev. C {\bf 56}, 954 (1997).
\bibitem{Bra88} M.E. Brandan and G.R. Satchler, Nucl. Phys. A {\bf 487}, 477 (1988).
\bibitem{Kho00a} D.T. Khoa, W. von Oertzen, H.G. Bohlen, and F. Nuoffer, 
	Nucl. Phys. A {\bf 672}, 387 (2000).
\bibitem{Mich01} F. Michel, G. Reidemeister, and S. Ohkubo, 
 Phys. Rev. C {\bf 63}, 034620 (2001).
\bibitem{Ohku14-1} S. Ohkubo and Y. Hirabayashi, Phys. Rev. C {\bf 89}, 051601(R) (2014).
\bibitem{Brau82} P. Braun-Munziger and J. Barette, Phys. Rep. {\bf 87}, 209 (1982).
\bibitem{Frahn80} W.E. Frahn and M.S. Hussein, Phys. Lett. {\bf 90B}, 358 (1980).
\bibitem{Frahn80s} W.E. Frahn and M.S. Hussein, Nucl. Phys. A {\bf 346}, 237 (1980).
\bibitem{Frahn84} W.E. Frahn, {\it Treaties on Heavy-Ion Science} vol.~1, p.~135, 
 ed. D.A. Bromley (Plenum Press, New York, 1984).
\bibitem{Phuc18} N.T.T. Phuc, N.H. Phuc, and D.T. Khoa, 
 Phys. Rev. C {\bf 98}, 024613 (2018).
\bibitem{vOe75} W. von Oertzen and H.G. Bohlen, Phys. Rep. {\bf 19 C}, 1 (1975).
\bibitem{Mor11} M.C. Morais and R. Lichtenth\"{a}ler, Nucl. Phys. A {\bf 857}, 1 (2011).
\bibitem{Hama11} Sh. Hamada, N. Burtebayev, K.A. Gridnev, and N. Amangeldi, 
 Nucl. Phys. A {\bf 859}, 29 (2011). 
\bibitem{Szi02} S. Szilner, W. von Oertzen, Z. Basrak, F. Haas, and M. Milin,
	Eur. Phys. J. A {\bf 13}, 273 (2002). 
\bibitem{Rud10} A.T. Rudchik {\it et al.}, Eur. Phys. J. A {\bf 44}, 221 (2010).
\bibitem{Raynal} J. Raynal, {\it Computing as a Language of Physics}
 (IAEA, Vienna, 1972) p.~75;  J. Raynal, coupled-channel code ECIS97 (unpublished).
\bibitem{Volya15} A. Volya and Y. M. Tchuvilsky, Phys. Rev. C {\bf 91}, 044319 (2015).
\bibitem{Yama12} T. Yamada, Y. Funaki, T. Myo, H. Horiuchi, K. Ikeda, G. R\"opke,
 P. Schuck, and A. Tohsaki, Phys. Rev. C {\bf 85}, 034315 (2012).
\bibitem{Tho88} I.J. Thompson, Comput. Phys. Rep. {\bf 7}, 167 (1988); 
 http://www.fresco.org.uk.
\bibitem{Tho09} I.J. Thompson and F.M. Nunes, {\it Nuclear Reactions for Astrophysics} 
(Cambridge University Press, Cambridge, UK, 2009).
\bibitem{Phuc19} N.T.T. Phuc, R.S. Mackintosh, N.H. Phuc, and D.T. Khoa, 
 Phys. Rev. C {\bf 100}, 054615 (2019).
\bibitem{Mack19} R.S. Mackintosh, Eur. Phys. J. A {\bf 55}: 147 (2019). 
\end{thebibliography}
